PTUM: Pre-training User Model from Unlabeled User Behaviors via Self-supervision

User modeling is critical for many personalized web services. Many existing methods model users based on their behaviors and the labeled data of target tasks. However, these methods cannot exploit useful information in unlabeled user behavior data, and their performance may be not optimal when labeled data is scarce. Motivated by pre-trained language models which are pre-trained on large-scale unlabeled corpus to empower many downstream tasks, in this paper we propose to pre-train user models from large-scale unlabeled user behaviors data. We propose two self-supervision tasks for user model pre-training. The first one is masked behavior prediction, which can model the relatedness between historical behaviors. The second one is next $K$ behavior prediction, which can model the relatedness between past and future behaviors. The pre-trained user models are finetuned in downstream tasks to learn task-specific user representations. Experimental results on two real-world datasets validate the effectiveness of our proposed user model pre-training method.

==> data/relatedwork.tex <==

\section{Related Work}\label{sec:RelatedWork}
%\subsection{User Modeling}
User modeling is a process that aims to build up a conceptual understanding of users~\cite{fischer2001user}.
It is an important technique for personalized web services such as personalized news, video and ad recommendation.
Many user methods incorporating other kinds of user information to enhance user representation learning, such as user behaviors and user profiles.
For example, Zhou et al.~\shortcite{zhou2018deep} proposed a deep interest network to learn user representations for CTR prediction based on the similarity between features extracted from candidate ads and user behaviors on e-commerce platforms.
Lian et al.~\shortcite{lian2018towards} proposed to learn user representations for news recommendation from the features extracted from user behaviors and profiles via a combination of  neural networks with different depths. 
However, these methods rely on handcrafted features to represent users, which requires massive expertise.


In recent years, there are several methods that learn user representations from the content of user behavior data such as texts~\cite{wang2018dkn,wu2019neural,zhu2019dan,an2019neural}.
For example, Wang et al.~\shortcite{wang2018dkn} proposed a news recommendation approach that learns news representations from news titles first via a knowledge-aware CNN, and learns user representations from the representations of browsed news articles according to their similarity with the candidate news representation.
Wu et al.~\shortcite{wu2019neural} proposed a hierarchical user representation with attention model for user demographic prediction, which learns search query representations from words and learns user representations from search queries.
They also use word-level and query-level attention networks to select important words and queries.
An et al.~\shortcite{an2019neural} proposed to use a multi-view learning framework to incorporate different kinds of user behaviors as different views of users, and use a view-level attention network to synthesize user representations learned from different views for ads CTR prediction.
In all aforementioned methods, user representations are learned based on the supervision in specific tasks, and the information of massive unlabeled user behavior data is not incorporated.
Different from these methods, our approach uses a user model pre-trained in a self-supervised manner to exploit useful information from unlabeled user behavior data, and experimental results show that our pre-trained user model can effectively improve the performance of downstream tasks such as user demographic prediction and CTR prediction.


\begin{comment}
\subsection{Pre-trained Language Model}
Recently, several pre-trained language models are proposed  and have made a great impact on  the NLP field~\cite{devlin2019bert,lan2019albert,yang2019xlnet}. 
For example,  Peters et al.~\shortcite{peters2018deep} proposed ELMo, which uses stacked LSTMs pre-trained in an autoregressive language modeling task to generate context-aware word embeddings.
Radford et al.~\shortcite{radford2018improving} proposed GPT, which can enhance the context modeling in a language model by using directional Transformers~\cite{vaswani2017attention} pre-trained in an autoregressive manner.
Devlin et al.~\shortcite{devlin2019bert} proposed BERT, which can capture the left and right contexts by using bidirectional Transformers, which are pre-trained in a masked token prediction task and a sentence pair classification task simultaneously.
Yang et al.~\shortcite{yang2019xlnet} proposed XLNET, which utilizes the Transformer-XL~\cite{dai2019transformer} architecture pre-trained in an autoregressive task by maximizing the expected log likelihood of all permutations of the factorization orders.
These pre-trained language models can learn universal language representations from large unlabeled corpus via self-supervision and can avoid training models from scratch in downstream tasks.
Similar to language models, a user model can also be pre-trained from unlabeled user behavior data in a self-supervised manner to have a universal understanding of users, which may benefit various downstream user-intensive tasks.
\end{comment}
